A hop away from everywhere: A view of the intercontinental long-haul infrastructure

Over the past two decades, a desire to reduce transit cost, improve control over routing and performance, and enhance the quality of experience for users, has yielded a more densely connected, flat network with fewer hops between sources and destinations. The shortening of paths in terms of the number of hops or links has also meant, for what is at the end an infrastructure-bound network, the lengthening of many of these links. In this paper, we focus on an important aspect of the evolving logical connectivity of the Internet that has received little attention to date: intercontinental long-haul links. We develop a methodology and associated processing system for identifying long haul links in traceroute measurements. We apply this system to a large corpus of traceroute data and report on multiple aspects of long haul connectivity including country-level prevalence, routers as international gateways, preferred long-haul destinations, and the evolution of these characteristics over a 7 year period. We identify over 9K layer 3 links that satisfy our definition for intercontinental long haul with many of them terminating in a relatively small number of nodes. An analysis of connected components shows a clearly dominant one with a relative size that remains stable despite a significant growth of the long-haul infrastructure.

==> tex/limitations.tex <==
\section{Limitations}\label{sec:limitations}

\begin{enumerate}
\item We have a limited visibility of the underlying infrastructure enabling long-haul connectivity. The widespread prevalence of MPLS and SD-WAN reduces even more our possibilities to extract topological characteristic from traceroute-derived analysis. However, in private conversation with operators affiliated to the SubOptic community, we obtain details that current trends in the use of physical infrastructure include network virtualization and other techniques to move the landing points inland to the proximity of datacenters. In a different context, a city-wide Internet outage in Cali Colombia after cable cut in a 100km segment that connects the city with the submarine cable landing point shows that long-haul connectivity is the result of consecutive segments of different physical technologies.
\item ICMP-unresponsive hops (Missing both sides of the LHL, Missing one side of the LHL (LHL defined as consecutive hops))
\item Packet loss in one sides of a route only traversed once
\item Geolocation inaccuracies (inherited from CAIDA's ITDK)
\item Eventual false positives in traceroute discontinuities
\item Pathological long delays in load balancers or firewalls (potentially fixed with geolocation)
\item Slow recurrent congestion (potentially fixed with geolocation)
\item  Limitations of the state-of-the-art alias resolution tools (False positives False negatives)
\item Limitations of the state-of-the-art router2asn mapping techniques (bdrmapit) e.g., inaccuracies in the AS routing mappings
\item Limited understanding of Organization-level routing and coordination due to limitations in AS2Org inferences
\begin{itemize}
\item Not only sibling ASes, also the parent-child relationships in a conglomerate (e.g., Orange, DTAC)
\item e.g., All ASes belonging to subsidiaries of the same organization peer at the same facility with the same upstream providers (CLARO)
\end{itemize}
\item Growth of the measurements platforms expanding to further unexplored locations (e.g., the developing world, Paraguay)
\item Biases of measurements platforms
\item Asymmetic paths making that distance between routers is actually shorter
\item Always growing networks prefixes and ASes (is this a problem)?
\item Inaccurate inter-hop latency jump. Near- and far-side router responses could take different reverse paths giving lower differences than the actual difference between roouters

\end{enumerate}•


==> tex/stability.tex <==
\begin{figure}[t!] 
\centering 
	\includegraphics[width=.4\textwidth]{fig/downsampling_nodes_edges.pdf}
	\caption{
	Fraction of LHL nodes (left) and edges (right) discovered when the number of traceroutes containing LHLs is downsampled.
% 	\vspace{-3mm}
	} \label{fig:data_samping}
\end{figure}

\section{Temporal stability and data convergence}

In this section we investigate the consistency and robustness of our observations relying on three different stability analyses: temporal stability (\S\ref{sec:stability:temp}), data convergence (\S\ref{sec:stability:convergence}), and threshold sensitivity (\S\ref{sec:stability:threshold}).

%****************************************
\subsection{Temporal stability}\label{sec:stability:temp}

Our initial analysis is based on a single traceroute measurement campaign collected by the CAIDA's Ark~\cite{ark}. While each of these campaigns or cycles is a network-wide topological exploration where vantage points probe all prefixes visible in BGP routing tables, each cycle is carried out over a single day. A question then is the stability of our observations over short time windows (days to weeks). We assume that the structure of the LHL network remains stable over short time windows given that it can be mainly affected by changes in commercial relationship between ASes, the deployment of new infrastructure, the large-scale network reallocations, all changes that move at a much slower pace and that take time to be put in place~\cite{paxson1997end, oliveira2009quantifying}.

% In Section~\ref{sec:longitudinal}, we include in all the analyses two snapshots of measurements collected in two consecutive weeks during 2020 ( measurement centered in cycles 8821 (2020 (1)) and 8839 (2020 (2))).
To validate this, we look at the LHL network using snapshots 2020 (1) and 2020 (2) that were collected during consecutive weeks. 
The temporal stability of values and distribution profiles of the long-haul network, which we analyzed in Sec.~\ref{sec:longitudinal}, allow us to gain confidence in the consistency of our observations and methodologies.
\ecnote{This last sentence should be more clear}


%****************************************
\subsection{Data convergence}\label{sec:stability:convergence}

In this section we explore the impact of using smaller, random subsets of a measurement campaign on the characteristics of the inferred long-haul network. For this, we look at the average fraction of nodes and edges of the long-haul network discovered when the number of traceroutes containing latency discontinuities is downsampled in powers of 2 ($<2, 4, 8, \dots, 512>$) in 100 runs with different randomly selected subsets.


\begin{figure}[t!] 
\centering 
	\includegraphics[width=.4\textwidth]{fig/threshold_sensitivity.pdf}
	\caption{
	Relative growth in number of nodes and edges for different values of the LHL threshold. In red is the LHL threshold used in our analysis.
	} \label{fig:sensitivity}
\end{figure}

Figure~\ref{fig:data_samping} shows the average fraction of nodes and edges of the long-haul network discovered for these different downsamplings rates. We observe that the number of nodes and edges remains almost the same when the number of candidates links drops by 2, and they drop 25\% when the downsampling increases to 4.
Moreover, when we select every other 16 traceroutes with discontinues, the number of nodes only drops to 0.5.
%These results shows that the long-haul network rapidly emerges with a few traceroutes and we suspect including extra measurement cycles would not substantially contribute to increase the visibility of the LHL network. We also observe a fairly small fluctuation in the number of nodes discovered in different random experiments where the coefficient of variation ($\sigma / \mu$) remained under 0.02 for all downsampling rates.
\textcolor{red}{
In the other way around, from a bottom-up perspective, these results shows that the long-haul network rapidly emerges with a few traceroutes and at the end of the process we observe that the long-haul network has converged since we double the number of traceroutes but this has little impact in the number of new nodes and edges discovered.
We suspect including extra measurement cycles would not substantially contribute to increase the visibility of the LHL network. 
We also observe a fairly small fluctuation in the number of nodes discovered in different random experiments where the coefficient of variation ($\sigma / \mu$) remained under 0.02 for all downsampling rates.
}


%****************************************
\subsection{Threshold sensitivity}\label{sec:stability:threshold}

Last, we carried out a sensitivity analysis of the latency threshold used in our definition of LHL (\S~\ref{sec:method:th}). The definition relies on a latency threshold which we have set to 40ms based on the distribution of distances between the largest peering facilities in each continent. We did a sensitivity analysis of this threshold focusing on changes to the long-haul network, both in terms of number of nodes and links. In our analysis we varied the threshold by $\pm$10ms (30 to 50ms), equivalent to 1864 to 3100 miles (with a latency bound of $\frac{4}{9}c$).




Figure~\ref{fig:sensitivity} shows changes in the fraction of nodes (left) and edges (right) of the resulting LHL network for the different thresholds. 
%We observe that changes of $\pm$10ms in the LHL threshold yields minor variations in both metrics - $\approx$7\% and $\approx$5\% in the number of nodes and edges, respectively, in the resulting LHL network.
\textcolor{red}{
Despite changes in the threshold do modify the number of routers and edges providing {\em international long-haul connectivity}, we observe that a threshold of 15ms (equivalent of the round-trip propagation delay between Buenos Aires and Santiago de Chile) adds 20\% more nodes and 15\% more edges.
On the other hand, a threshold of 65ms (equivalent of the round-trip propagation delay between New York City and Frankfurt) reduces 12\% of the nodes and 8\% of the edges.
We recall the distance analysis between countries' capital cities (Sec) and 16\% more capital cities are included when when reduce the threshold from 40 to 15 and 21\% are excluded when increase the threhold up to 65ms.
}






